Differentially Private Active Learning: Balancing Effective Data Selection and Privacy

Active learning (AL) is a widely used technique for optimizing data labeling in machine learning by iteratively selecting, labeling, and training on the most informative data. However, its integration with formal privacy-preserving methods, particularly differential privacy (DP), remains largely underexplored. While some works have explored differentially private AL for specialized scenarios like online learning, the fundamental challenge of combining AL with DP in standard learning settings has remained unaddressed, severely limiting AL's applicability in privacy-sensitive domains. This work addresses this gap by introducing differentially private active learning (DP-AL) for standard learning settings. We demonstrate that naively integrating DP-SGD training into AL presents substantial challenges in privacy budget allocation and data utilization. To overcome these challenges, we propose step amplification, which leverages individual sampling probabilities in batch creation to maximize data point participation in training steps, thus optimizing data utilization. Additionally, we investigate the effectiveness of various acquisition functions for data selection under privacy constraints, revealing that many commonly used functions become impractical. Our experiments on vision and natural language processing tasks show that DP-AL can improve performance for specific datasets and model architectures. However, our findings also highlight the limitations of AL in privacy-constrained environments, emphasizing the trade-offs between privacy, model accuracy, and data selection accuracy.

==> figs/algs/algs_combines.tex <==
\begin{figure*}[t]
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \input{figs/algs/naive_dpal.tex}
        \caption{\emph{Naive} active learning with DP-SGD. \texttt{get\_noiseMultiplier} is an Opacus function that compute the noise multiplier given some privacy parameters using binary search \cite{Yousefpour2021}. \texttt{DP-SGD} is a function that trains a model for a given number of steps using DP-SGD.}
        \label{alg:al}
    \end{minipage}%
    \hspace{0.5cm}%
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \input{figs/algs/dpal.tex}
          \caption{Binary search algorithm for \emph{step amplification}. $n_{:i}$ denotes the number of training steps until iteration $i$. \texttt{get\_epsilon} is an Opacus function that computes the privacy loss from DP-SGD training \cite{Yousefpour2021}. \texttt{get\_sampleRate} is a function that computes the sampling rate corresponding to the given privacy parameters using a similar binary search algorithm \cite{Boenisch2023b}.}
         \label{alg:stepampl}
    \end{minipage}
\end{figure*}
